Regularising NARX models with multi-task learning

A Nonlinear Auto-Regressive with eXogenous inputs (NARX) model can be used to describe time-varying processes; where the output depends on both previous outputs and current/previous external input variables. One limitation of NARX models is their propensity to overfit and result in poor generalisation for future predictions. The proposed method to help to overcome the issue of overfitting is a NARX model which predicts outputs at both the current time and several lead times into the future. This is a form of multi-task learner (MTL); whereby the lead time outputs will regularise the current time output. This work shows that for high noise level, MTL can be used to regularise NARX with a lower Normalised Mean Square Error (NMSE) compared to the NMSE of the independent learner counterpart.

==> References.tex <==
@article{Bee2024,
   title={When is an \uppercase{SHM} problem a Multi-Task-Learning problem?},
   author={S.C. Bee and L.A. Bull and N. Dervilis and K. Worden},
   journal={arXiv preprint arXiv:2305.09425},
   year={2023}
}

@article{Butterworth1930,
  title = {On the Theory of Filter Amplifiers},
  volume = {7},
  journal = {Experimental Wireless \& the Wireless Engineer},
  author = {Butterworth, S.},
  month = oct,
  year = {1930},
  pages = {536-541}
}

@article{caruana1997,
abstract = {Multitask Learning is an approach to inductive transfer that improves generalization by using the domain information contained in the training signals of related tasks as an inductive bias. It does this by learning tasks in parallel while using a shared representation; what is learned for each task can help other tasks be learned better. This paper reviews prior work on MTL, presents new evidence that MTL in backprop nets discovers task relatedness without the need of supervisory signals, and presents new results for MTL with k-nearest neighbor and kernel regression. In this paper we demonstrate multitask learning in three domains. We explain how multitask learning works, and show that there are many opportunities for multitask learning in real domains. We present an algorithm and results for multitask learning with case-based methods like k-nearest neighbor and kernel regression, and sketch an algorithm for multitask learning in decision trees. Because multitask learning works, can be applied to many different kinds of domains, and can be used with different learning algorithms, we conjecture there will be many opportunities for its use on real-world problems.},
author = {Caruana, Rich},
doi = {10.1023/A:1007379606734},
file = {:C$\backslash$:/Users/scbee/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Caruana - 1997 - Multitask Learning.pdf:pdf},
issn = {1573-0565},
journal = {Machine Learning },
keywords = {Artificial Intelligence,Control,Mechatronics,Natural Language Processing (NLP),Robotics,Simulation and Modeling},
number = {1},
pages = {41--75},
publisher = {Springer},
title = {{Multitask Learning}},
volume = {28},
year = {1997}}

@article{Champneys2022,
title = {On the dynamic properties of statistically-independent nonlinear normal modes},
journal = {Mechanical Systems and Signal Processing},
volume = {181},
pages = {109510},
year = {2022},
issn = {0888-3270},
doi = {https://doi.org/10.1016/j.ymssp.2022.109510},
author = {M.D. Champneys and G. Tsialiamanis and T.J. Rogers and N. Dervilis and K. Worden},
keywords = {Nonlinear normal modes, Nonlinear system identification, Machine learning, cycle-GAN, Higher-order frequency-response functions},
abstract = {Much attention has been given to the study of nonlinear normal modes (NNMs), a nonlinear extension to the eminently useful framework for the analysis of linear dynamics provided by linear modal analysis (LMA). In the literature, several approaches have gained traction, with each able to preserve a subset of the useful properties of LMA. A recently-proposed framework (Worden and Green, 2017) casts nonlinear modal analysis as a problem in machine learning, viewing the NNM as directions in a latent modal coordinate space within which the modal dynamics are statistically uncorrelated. Thus far, the performance of this framework has been measured in a largely qualitative way. This paper presents, for the first time, an exploration into the underlying dynamics of the statistically-independent NNMs using techniques from nonlinear system identification (NLSI) and higher-order frequency-response functions (HFRFs). In this work, the statistically-uncorrelated NNMs are found for two simulated nonlinear cubic-stiffness systems using a recently-proposed neural-network based approach. NLSI models are fitted to both physical and modal displacements and the HFRFs of these models are compared to theoretical values. In particular, it is found for both systems that the modal decompositions here permit an independent single-input single-output (SISO) representation that can be projected back onto the original displacements with low error. It is also shown via the HFRFs that the underlying linear natural frequencies of the modal dynamics lie very close to the underlying linear natural frequencies of the nonlinear systems, indicating that a true nonlinear decomposition has been identified.}
}

@article{Chance1998,
title = {FREQUENCY DOMAIN ANALYSIS OF \uppercase{NARX} NEURAL NETWORKS},
journal = {Journal of Sound and Vibration},
volume = {213},
number = {5},
pages = {915-941},
year = {1998},
issn = {0022-460X},
doi = {https://doi.org/10.1006/jsvi.1998.1539},
author = {J.E. Chance and K. Worden and G.R. Tomlinson},
abstract = {A method is proposed for interpreting the behaviour of NARX neural networks. The correspondence between time-delay neural networks and Volterra series is extended to the NARX class of networks. The Volterra kernels, or rather, their Fourier transforms, are obtained via harmonic probing. In the same way that the Volterra kernels generalize the impulse response to non-linear systems, the Volterra kernel transforms can be viewed as higher-order analogues of the Frequency Response Functions commonly used in Engineering dynamics; they can be interpreted in much the same way.}
}

@article{Hernández-González2024,
title = {\uppercase{AI}-driven blind source separation for fast operational modal analysis of structures},
journal = {Mechanical Systems and Signal Processing},
volume = {211},
pages = {111267},
year = {2024},
issn = {0888-3270},
doi = {https://doi.org/10.1016/j.ymssp.2024.111267},
author = {Israel Alejandro Hernández-González and Enrique García-Macías and Gabriele Costante and Filippo Ubertini},
keywords = {Artificial intelligence, Blind source identification, Damage identification, Deep Neural Networks, Operational Modal Analysis, Structural Health Monitoring},
abstract = {The management of the aging built infrastructure stands as a paramount concern on the political agendas worldwide, bearing far-reaching socio-economic impacts. The growing trend of tragic collapses in recent years underscore the urgent need for efficient structural health maintenance (SHM) strategies to support decision-making in prioritizing intervention and rehabilitation actions. Vibration-based SHM systems utilizing Operational Modal Analysis (OMA) have gained popularity owing to their non-destructive nature, global damage assessment capabilities, and relatively straightforward automation with minimal intrusiveness. Nevertheless, state-of-the-art OMA techniques often face significant scalability limitations, primarily driven by extensive computational requirements and need for substantial expert involvement. In this context, recent advances in the realm of artificial intelligence (AI) offer great promise in addressing these scalability issues, paving the way for next-generation SHM systems. In this light, this work introduces a novel Multitask Learning Deep Neural Network (MTL-DNN) model designed for fast and automated blind source modal identification of structures. By encapsulating the principles of second-order blind source identification (SOBI) within the network’s architecture, the proposed model can extract the complex-valued modal components concealed within input raw response acceleration data. This enables the direct extraction of complex-valued mode shapes from the weights of the network, and the corresponding resonant frequencies and damping ratios are estimated through a computationally light single-degree-of-freedom identification algorithm. The efficacy of the presented approach is validated through three case studies: a theoretical non-proportionally damped system, a laboratory steel frame structure, and a real-world reinforced concrete arch bridge. The presented results demonstrate the capability of the proposed technique to conduct near-instantaneous automated modal identification with minimal expert intervention, holding great potential as a scalable technique for SHM of large infrastructural systems.}
}

@INPROCEEDINGS{Nikentari2022,
  author={Nikentari, Nerfita and Wei, Hua-Liang},
  booktitle={2022 27th International Conference on Automation and Computing (ICAC)}, 
  title={Multi-Task Learning for Time Series Forecasting Using \uppercase{NARMAX-LSTM}}, 
  year={2022},
  volume={},
  number={},
  pages={1-6},
  keywords={Knowledge engineering;Automation;Computational modeling;Time series analysis;Neural networks;Predictive models;Multitasking;multitask learning;NARMAXx;LSTM;forecasting},
  doi={10.1109/ICAC55051.2022.9911071}}


@article{Shu2023,
title = {A multi-task learning-based automatic blind identification procedure for operational modal analysis},
journal = {Mechanical Systems and Signal Processing},
volume = {187},
pages = {109959},
year = {2023},
issn = {0888-3270},
doi = {https://doi.org/10.1016/j.ymssp.2022.109959},
author = {Jiangpeng Shu and Congguang Zhang and Yifan Gao and Yanbo Niu},
keywords = {Structural heath monitoring, Artificial intelligence, Automatic blind identification, Multi-task deep neural network, Long-span bridge},
abstract = {Traditional modal analysis approaches for structural heath monitoring (SHM) have a low implementation efficiency. This study develops an artificial intelligence (AI)-based automatic blind identification procedure for determining the modal parameters of structures. The core of this procedure is to establish a multi-task deep neural network (MTDNN) that can automatically and efficiently extract independent modes from multi-mode vibration responses of structures. Then modal frequencies and damping ratios of structures can be extracted from independent modes via employing the conventional random decrement technique (RDT) and curve fitting approach. The weights between the last two layers of MTDNN represents the corresponding mode shapes. The approach is verified by a five-degree-of-freedom numerical model and then implemented to a field test of a long-span cable-stayed bridge in engineering practice. The results indicate the ability of the developed approach to automatically determine the modal parameters of structures with reliable accuracy. In the prediction stage, the modal separation process by using MTDNN takes only about 0.12 s (numerical example) and 0.48 s (practical example). The computational efficiency of the developed approach is significantly higher than that of traditional stochastic subspace identification (SSI) and frequency domain decomposition (FDD) approaches, which provides a promising new solution for online modal parameter identification and modal tracking of structures.}
}


@article{Tu2023,
author = {X.L. Tu and R.J. Pyle and A.J. Croxford and P.D. Wilcox},
title ={Potential and limitations of \uppercase{NARX} for defect detection in guided wave signals},
journal = {Structural Health Monitoring},
volume = {22},
number = {3},
pages = {1863-1875},
year = {2023},
doi = {10.1177/14759217221113240},
abstract = { Previously, a nonlinear autoregressive network with exogenous input (NARX) demonstrated an excellent performance, far outperforming an established method in optimal baseline subtraction, for defect detection in guided wave signals. The principle is to train a NARX network on defect-free guided wave signals to obtain a filter that predicts the next point from the previous points in the signal. The trained network is then applied to new measurement and the output subtracted from the measurement to reveal the presence of defect responses. However, as shown in this paper, the performance of the previous NARX implementation lacks robustness; it is highly dependent on the initialisation of the network and detection performance sometimes improves and then worsens over the course of training. It is shown that this is due to the previous NARX implementation only making predictions one point ahead. Subsequently, it is shown that multi-step prediction using a newly proposed NARX structure creates a more robust training procedure, by enhancing the correlation between the training loss metric and the defect detection performance. The physical significance of the network structure is explored, allowing a simple hyperparameter tuning strategy to be used for determining the optimal structure. The overall detection performance of NARX is also improved by multi-step prediction, and this is demonstrated on defect responses at different times as well as on data from different sensor pairs, revealing the generalisability of this method. }
}

@article{Urbani1994,
  author={Urbani, D. and Roussel-Ragot, P. and Personnaz, L. and Dreyfus, G.},
  booktitle={Proceedings of IEEE Workshop on Neural Networks for Signal Processing}, 
  title={The selection of neural models of nonlinear dynamical systems by statistical tests}, 
  year={1994},
  volume={},
  number={},
  pages={229-237},
  keywords={Nonlinear dynamical systems;System testing;Predictive models;Neural networks;Context modeling;Multi-layer neural network;Polynomials;Structural engineering;Reduced order systems;Recurrent neural networks},
  doi={10.1109/NNSP.1994.366044}}


@article{Wan2022,
title = {An improved complex multi-task \uppercase{B}ayesian compressive sensing approach for compression and reconstruction of \uppercase{SHM} data},
journal = {Mechanical Systems and Signal Processing},
volume = {167},
pages = {108531},
year = {2022},
issn = {0888-3270},
doi = {https://doi.org/10.1016/j.ymssp.2021.108531},
author = {Hua-Ping Wan and Guan-Sen Dong and Yaozhi Luo and Yi-Qing Ni},
keywords = {Bayesian compression sensing, Complex-valued domain, Multi-task learning, Discrete Fourier basis, Structural health monitoring (SHM)},
abstract = {The long-term structural health monitoring (SHM) provides massive data, leading to a high demand for data transmission and storage. Compressive sensing (CS) has great potential in alleviating this problem by using less samples to recover the complete signals utilizing the sparsity. Vibration data collected by an SHM system is usually sparse in the frequency domain, and the peaks in their Fourier spectra most often correspond to the same frequencies. This underlying commonality among the signals can be utilized by multi-task learning technique to improve the computational efficiency and accuracy. While being real-valued originally, the data after discrete Fourier transformation are in general complex-valued. In this paper, an improved complex multi-task Bayesian CS (CMT-BCS) method is developed for compression and reconstruction of SHM data requiring a high sampling rate. The novelty of the proposed method is twofold: (i) it overcomes the invalidity of the conventional CMT-BCS approach in dealing with the ‘incomplete’ CS problem, and (ii) it improves the computational efficiency of conventional CMT-BCS approach. The former is achieved by restructuring the CMT-BCS formulation, and the latter is realized by sharing a common sampling matrix across all tasks of concern. The improved CMT-BCS is evaluated using the shaking table test data of a scale-down frame model and the real-world SHM data acquired from a supertall building. A comparison with several existing BCS methods that enable to deal with complex values is also provided to demonstrate the effectiveness of the proposed method.}
}

@article{Worden2007,
title = {Identification of pre-sliding and sliding friction dynamics: Grey box and black-box models},
journal = {Mechanical Systems and Signal Processing},
volume = {21},
number = {1},
pages = {514-534},
year = {2007},
issn = {0888-3270},
doi = {https://doi.org/10.1016/j.ymssp.2005.09.004},
author = {K. Worden and C.X. Wong and U. Parlitz and A. Hornstein and D. Engster and T. Tjahjowidodo and F. Al-Bender and D.D. Rizos and S.D. Fassois},
abstract = {The non-linear dependence of pre-sliding and sliding friction forces on displacement and velocity is modelled using different physics-based and black-box approaches including various Maxwell-Slip models, neural networks, non-parametric (local) models and recurrent networks. The efficiency and accuracy of these identification methods is compared for an experimental time series where the observed friction force is predicted from the measured displacement and estimated velocity. All models, although varying in their degree of accuracy, show good prediction capability of friction. Finally, it is shown that better results can be achieved by using an ensemble of the best models for prediction.}
}

@book{Worden2019,
  title={Nonlinearity in Structural Dynamics: Detection, Identification and Modelling},
  author={Worden, K. and Tomlinson, G.},
  isbn={9780429524981},
  year={2019},
  publisher={CRC Press},
  pages = {52}
}

@article{Xue2023,
title = {Damage localization and robust diagnostics in guided-wave testing using multitask complex hierarchical sparse Bayesian learning},
journal = {Mechanical Systems and Signal Processing},
volume = {197},
pages = {110365},
year = {2023},
issn = {0888-3270},
doi = {https://doi.org/10.1016/j.ymssp.2023.110365},
author = {Shicheng Xue and Wensong Zhou and James L. Beck and Yong Huang and Hui Li},
keywords = {Nondestructive testing, Damage localization, Robust diagnosis, Guided wave, Bayesian uncertainty quantification, Complex hierarchical sparse Bayesian learning},
abstract = {The inversion of guided-wave data for accurate damage localization is a challenging problem when using guided waves for nondestructive testing and robust diagnostics. It is especially important to detect incorrect damage localization without knowing the original damage. In this paper, a new damage localization and robust diagnostics method is proposed. A Multi-task Complex Hierarchical Sparse Bayesian learning (MuCHSBL) algorithm is presented to solve the inverse problem for damage localization based on the data measured from a small number of sensors. The multi-task model improves the efficacy of damage localization by utilizing the consistency of damage locations for tasks with different signal frequencies. A Sparse Bayesian learning algorithm is also introduced to utilize the spatial sparsity of the damage, since structural damage typically occurs at only a few localized areas. The quantified posterior uncertainty of the model parameters gives a sense of confidence in the damage localization results. Utilizing the different levels of uncertainty in the optimal and suboptimal inversion models, diagnostic tools are proposed to detect whether the inversion for damage localization is accurate, without knowing the original damage. Numerical and experimental studies are carried out to verify the effectiveness of the proposed method. It is demonstrated that the damage localization efficacy of multi-task model is much higher than that of single-task model; moreover, the accuracy of damage localization results can be diagnosed effectively by the posterior uncertainty quantification of the model parameters.}
}


